A Management Framework for Secure Multiparty Computation in Dynamic Environments

Secure multiparty computation (SMC) is a promising technology for privacy-preserving collaborative computation. In the last years several feasibility studies have shown its practical applicability in different fields. However, it is recognized that administration and management overhead of SMC solutions are still a problem. A vital next step is the incorporation of SMC in the emerging fields of the Internet of Things and (smart) dynamic environments. In these settings, the properties of these contexts make utilization of SMC even more challenging since some of its vital premises regarding environmental stability and preliminary configuration are not initially fulfilled. We bridge this gap by providing FlexSMC, a management and orchestration framework for SMC which supports the discovery of nodes, supports a trust establishment between them and realizes robustness of SMC session by handling nodes failures and communication interruptions. The practical evaluation of FlexSMC shows that it enables the application of SMC in dynamic environments with reasonable performance penalties and computation durations allowing soft real-time and interactive use cases.

==> Makefile <==
FILENAME = "ieeetrans_paper"

pdf:
	- pdflatex $(FILENAME).tex
	- bibtex $(FILENAME).aux
	- pdflatex $(FILENAME).tex
	- pdflatex $(FILENAME).tex
#	- pdftotext -nopgbrk -raw $(FILENAME).pdf - | grep -i --color TODO


clean:
	- find . | egrep ".*((\.(pdfsync|aux|idx|ind|ilg|log|blg|bbl|toc|lof|lot|dvi|tlf|tlt|glo|out|tcp|nlo|nls|glo|gls|acn|acr|alg|glg|ist|loa|synctex.gz))|~)$$" | xargs rm
	- rm -f $(FILENAME)-blx.bib
	- rm -f $(FILENAME).pdf
	- rm -f $(FILENAME).run.xml
	- rm -f $(FILENAME).synctex.gz
	- rm -f $(FILENAME).xdy
	- rm -f $(FILENAME).ent


#end of Makefile




==> latexmkrc <==
add_cus_dep( 'glo', 'gls', 0, 'makeglossaries' );
sub makeglossaries {
  system( "makeglossaries \"$_[0]\"" );
}



